AI-enhanced semantic feature norms for 786 concepts

Semantic feature norms have been foundational in the study of human conceptual knowledge, yet traditional methods face trade-offs between concept/feature coverage and verifiability of quality due to the labor-intensive nature of norming studies. Here, we introduce a novel approach that augments a dataset of human-generated feature norms with responses from large language models (LLMs) while verifying the quality of norms against reliable human judgments. We find that our AI-enhanced feature norm dataset, NOVA: Norms Optimized Via AI, shows much higher feature density and overlap among concepts while outperforming a comparable human-only norm dataset and word-embedding models in predicting people's semantic similarity judgments. Taken together, we demonstrate that human conceptual knowledge is richer than captured in previous norm datasets and show that, with proper validation, LLMs can serve as powerful tools for cognitive science research.

==> intro_orig.tex <==
Beginning from classical exemplar theoretic accounts of categorization to connectionist models of semantic knowledge, a persistent view has been that concepts are organized in terms of the properties or features that they possess.
For example, groups of concepts that have largely overlapping sets of features help define broader semantic categories and the precise degree to which features overlap help determine the typicality of the concept within that category \cite{rosch1975cognitive}.
Research in this domain has been facilitated using \textit{semantic norm} datasets, which are generated by having people list features that they know to be true for a given concept.
By aggregating listed features across many subjects, it is possible to create vector representations of concepts (often referred to as semantic vectors), where the dimensions of the vectors correspond to the elicited features.
Many such norm datasets have been collected over the years \citep{mcrae2005semantic, devereux2014centre, buchanan2019english, ruts2004dutch, hansen2022semantic}, and have been critical in answering questions relating to the organization and degradation of semantic memory \citep{collins1975spreading, collins1969retrieval,mcclelland2003parallel,ashcraft1978property, garrard2001longitudinal}.
A critical finding from \textcite{rosch1975family}, one of the earliest studies to employ semantic feature listing to create a bespoke norm dataset, was that what distinguished members within categories were the features that were ``true of some, but not all'' members.
That is, they found that many concepts, within the small set that they studied, possessed largely overlapping features and it was necessary to identify the few features that were \textit{not} true for all concepts in order to understand their organization.
Thus, to fully characterize the space of human semantic knowledge it is important to have a large representative set of features that both distinguish members of a category but also distinguish individual items within categories.

A primary limitation of many existing norm datasets, despite the considerable labor that goes into constructing them, is that they are nevertheless limited in terms of either the number of concepts included, the set of features represented, or both.
For example, the McRae norms \citep{mcrae2005semantic}, a well established dataset contains 541 concepts and  2,526 features. 
While this constitutes a reasonably large set of concepts, the limited number of unique features makes it unlikely that this dataset captures the full diversity of features that people represent in semantic memory.
Following up on this dataset, the Centre for Speech, Language and the Brain (CSLB) norms increased the number of concepts to 638 while also getting a higher average number of features listed per concept. They found that the average distinctiveness of concepts (number of features shared with other concepts) was lower in their dataset relative to the McRae norms highlighting the importance of getting high throughput feature listing data in order to uncover feature overlaps between concepts.
\citeauthor{buchanan2019english} (\citeyear{buchanan2019english}) further developed a large-scale feature norm corpus of over 4,000 concepts that consisted of not only nouns but concepts belonging to other parts of speech as well (although 70\%) were still nouns.
\citeauthor{hansen2022semantic} (\citeyear{hansen2022semantic}) used GPT-3's ability to generate text in response to human queries to generate a set of feature norms for the 1,854 THINGS \cite{hebart2022things} concepts resulting in a dataset with 11,683 unique machine generated features.
Another critical limitation of the semantic feature listing approach is that since some features might appear more `salient' to participants relative to others, many norm datasets underestimate the degree to which there is feature overlap between concepts. As an example, while the feature `is made of wood' can be true for both a `desk' and a `flute', people are more likely to list the feature for the former than the latter. This was addressed in the Leuven semantic norms \citep{de2008exemplar}, where the authors performed an additional ``applicability'' verification step where they asked a cohort of participants to verify all possible feature-concept pairings for the norms dataset collected by \textcite{ruts2004dutch}. This allowed for the generation of a more representative semantic norm dataset, however they restricted their applicability procedure to broad domains of concepts (animals and artifacts) thus limiting their ability to capture critical cross-domain structure. As it stands, this verification procedure is the most suitable method for obtaining high-quality semantic norms; however, it is labor-intensive and costly, which limits its scalability for creating large-scale datasets.

The recent rapid development of large language models (LLMs), such as OpenAI's GPT family of models \cite{openai-gpt4}, that can respond to human queries using natural language presents a potential way forward for developing a robust semantic norm dataset.
These models have been shown to broadly approximate various facets of human language and behavior \citep{bubeck2023sparks}, are capable of performing a variety of cognitive psychology experiments \cite{binz2023using,webb2023emergent} and capturing patterns of responses for behavioral experiments generally \citep{aher2023using}.
These results suggest that beyond simple next-token prediction, these models might reasonable understand the meanings of words and the concepts they refer to \citep{piantadosi2022meaning}, often raising provocative questions surrounding whether, on average, their performance might replace the efforts of human participants \citep{dillion2023can} (cf.\citep{mitchell2023we}).
While we don't take such a strong stance, we nevertheless believe language models in conjunction with human efforts might make tractable the problem of generating a large-scale semantic norm dataset, which does not compromise on feature verification. 
Such a norm would allow for ... \km{@Sid try and finish this}



%In developing a new semantic norms dataset, our first step was compiling a comprehensive list of 786 concepts, encompassing items from established datasets such as the McRae Norms, Ecoset, and Leuven Norms. This collection includes basic-level categories like ``dog'' and ``plant'', as well as superordinate categories such as``Animal'' and ``Bird''.

%Our workflow involves multiple stages of data collection, validation, and augmentation to construct a norms dataset that integrates both human-generated and AI-enhanced matrices. Initially, features were crowd-sourced for approximately 786 concepts, yielding around 25,000 unique features. Through clustering, this was reduced to 20,000 features, forming the human-generated matrix. A random subset of 10,000 concept-feature pairs was selected for human validation, where annotators provided true/false judgments, resulting in the human-judged validation set, which included 786 concepts and about 8,200 unique features.

%To investigate if we could use AI for feature verification, we evaluated various LLM-generated responses to these validation questions, selecting the strategy with the best d-prime performance against human judgments. Using this optimized approach, the LLMs were prompted to provide yes/no answers for all 8,200 features across all 786 concepts, creating the AI-augmented matrix—a binary matrix where each cell denotes the presence or absence of a feature for a given concept.

%For a structured comparison, we aligned the human-generated matrix with the AI-augmented matrix by filtering out any features absent in the AI-augmented set, producing the reduced human-generated matrix (786 concepts × 8,200 features). Unlike the sparse human-judged validation set, this matrix is fully populated with binary values, capturing all features originally elicited from humans. The final AI-augmented matrix which we release maintains the human-provided features while introducing additional ones inferred by the LLMs.

%Figure \ref{fig:schematic} illustrates this pipeline, highlighting the sequential transformations—from raw crowd-sourced data to feature reduction, validation, and AI augmentation.


%contained a higher number of features per concept compared to the human-only matrix. Additionally, concepts in the AI-enhanced matrix shared more features with one another than those in the human matrix (Figure \ref{fig:heatmap_stats}A). Ostensibly, this might seem to be the result of the LLM responding with `true' more frequently than it should leading to potential false positives. However, since the goal of the verification process was to also reveal feature overlap where it was absent we visualized the category selectivity of the embeddings by computing the cosine dissimilarity between pairs of concepts and sorting them by higher order categories derived from a combination of existing norm datasets and further LLM annotation. This can be seen in Figure \ref{fig:heatmap_stats} B for both the human only and AI-enhanced matrix.  Overall the similarity between all concepts increased indicated by the overall darker color of the AI-enhanced matrix. However, the category structure seen in the human only matrix was not only preserved in the AI-enhanced matrix but was further enhanced, indicating that while the verification process uncovered true category level similarity between concepts.



==> intro_ttr.tex <==
Semantic feature norms have been critical to the study of human conceptual knowledge since Rosch introduced them in the 1970's~\cite{rosch1975cognitive}. In norming tasks, participants list features they believe to be true of a given concept. Aggregating the features listed by many participants across a large set of concepts creates semantic vectors whose elements correspond to the elicited features, and whose entries indicate whether a given concept is commonly judged to possess the corresponding property. Rosch observed that proximity between two such feature vectors relates systematically to their perceived semantic relatedness---thus lions and tigers are viewed as similar kinds of things because they have many overlapping and few distinguishing properties. Norming datsets collected over the years \citep{mcrae2005semantic, devereux2014centre, buchanan2019english, ruts2004dutch, hansen2022semantic,dilkina2008semantic} have helped to answer questions about the organization semantic memory \citep{collins1975spreading,ashcraft1978property,}, its degradation in semantic disorders \citep{farahmcclelland1995,rogersETAL2004, garrard2001longitudinal,creemcraeXX,giallanzaETAL2024}, and its neural bases \cite{CoxETAL2024}.

Semantic norming requires extensive human labor both in data collection and curation/post-processing. Prior studies have met this challenge in different ways, each requiring some degree of compromise as elaborated below. Other recent work has sought alternatives to human feature norms by making use of natural language processing technologies, including word embeddings from methods such as GLOVE or word2vec \cite{XX} as well as feature norms generated artificially using large language models \citep{hansen2022semantic}). Both alternatives have their own drawbacks, however: it is not clear that word embeddings capture the semantic structure that humans perceive as well as do feature norms, at least for concrete objects \cite{XX}; and large language models can generate super-human lists of features that go far beyond what a typical person might know while simultaneously confabulating properties that are untrue \cite{XX}.

The current work seeks a middle way between human-only and machine-only norm generation. We crowd-sourced feature lists for a modestly large and representative set of 786 concrete object concepts, ensuring that the features included in the set are those that human participants discern in the task. We then used large language models to aid in the most labor-intensive parts of data curation and post-processing--feature reduction and feature verification--resulting in a novel {\em AI-enhanced} set of semantic feature norms. We illustrate remarkable differences between human-only and AI-enhanced norm sets, then report empirical studies designed to assess whether the AI-enhanced norms better capture human-perceived structure than do human-only norms or out-of-the-box word embeddings.


